Verifying Global Two-Safety Properties in Neural Networks with Confidence

We present the first automated verification technique for confidence-based 2-safety properties, such as global robustness and global fairness, in deep neural networks (DNNs). Our approach combines self-composition to leverage existing reachability analysis techniques and a novel abstraction of the softmax function, which is amenable to automated verification. We characterize and prove the soundness of our static analysis technique. Furthermore, we implement it on top of Marabou, a safety analysis tool for neural networks, conducting a performance evaluation on several publicly available benchmarks for DNN verification.

==> extra.tex <==
%\subsection{Hyper-Properties}

\emph{Global robustness}
\begin{multline*}
    \forall x, x', where \hspace{5pt} \epsilon>0, \exists \delta>0 \hspace{5pt} s.t. \hspace{2pt} |x - x'| \le \delta \\ \implies |f(x) - f(x')| \leq \epsilon
\end{multline*}
\emph{Global robustness with confidence}
\begin{multline*}
\forall x, x', where \hspace{5pt} \epsilon>0, \exists \delta>0 \hspace{5pt} s.t. \hspace{2pt} |x - x'| \le \delta \land conf(f(x))>k \\ \implies |f(x) - f(x')| \leq \epsilon 
\end{multline*}

However, softmax being a non-linear activation function cannot be used directly in our case. Hence, we approximate it as a linear function $\sigma'$. We denote this approximated confidence by $conf'(f(X\textsubscript i))$.

Let $f(\vec{x}) = \conf(g(\vec{x}))$ be a NN, where $g$ models the hidden layers and $\conf$ is the confidence softmax layer. We say that the NN $f$ is \emph{$k$-confidently $\delta$-robust} if 

For a DNN $N$, we use $n$ to denote the number of layers. Layer $1$ is the input layer, layer $n$ is the output layer and layers $2,\dotsc ,n-1$ are the hidden layers. The output, denoted by $Y\textsubscript i$ is calculated by propagating the input $X\textsubscript i$ through the network using predefined weights and biases, and applying the activation functions. Let this operation of finding the outputs given the inputs be denoted by $f(x)$ i.e., $ Y\textsubscript i = f(X\textsubscript i)$. 

Applying Softmax function $\sigma$ to $Y\textsubscript i$, gives $\sigma(Y\textsubscript i)$, which is the confidence with which outputs are predicted by $N$. 

As neural networks enter safety-critical applications such as healthcare, autonomous vehicles, and financial systems, the need for verifying their correctness and safety has become essential. It has been observed that neural networks can be opaque and difficult to understand, making it challenging to predict their behavior.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Softmax}
\subsubsection{Approximating softmax as a max operator and a sigmoid}
Let $\sigma (\overrightarrow z)\textsubscript i$
be the softmax function s.t.,
\begin{equation} \label{sigmoid_definition}
\sigma (\overrightarrow z)\textsubscript i = \frac{e^{z \textsubscript i}}{\sum_{j=1}^{N} e^{z\textsubscript j}}
\end{equation}

\noindent{Let us first establish the relationship between softmax and sigmoid. 
Consider ${\sigma (\overrightarrow z)\textsubscript i}$, for i=1,}
%\begin{equation} \label{sigma_for_i=1}
\begin{equation} \label{sigma_for_i=1}
\begin{split}
{\sigma (\overrightarrow z)\textsubscript 1} = \frac{e^{z {\textsubscript{\tiny 1}}}}{e^{z{\textsubscript{\tiny 1}}} + e^{z\textsubscript\tiny 2} + \dotsb + e^{z\textsubscript\tiny m} } = \frac{1}{1+ (e^{z{\textsubscript{\tiny 2}}} + \dotsb + e^{z{\textsubscript{\tiny m}}})e^{-z{\textsubscript{\tiny 1}}} } \\= \frac{1}{1+ e^{log (e^{z{\textsubscript{\tiny 2}}} + \dotsb + e^{z{\textsubscript{\tiny m}}})}e^{-z{\textsubscript{\tiny 1}}}} = \frac{1}{1+ e^{(-z{\textsubscript{\tiny 1}} + log (e^{z{\textsubscript{\tiny 2}}} + \dotsb + e^{z{\textsubscript{\tiny m}}}))}}
\end{split}
\end{equation}

We can now generalize the result from (\ref{sigma_for_i=1}) for i
\begin{equation} \label{sig_as_logsum}
\sigma (\overrightarrow z)\textsubscript i = \frac{1}{1+ e^{(-z{\textsubscript{\tiny i}} + log (\sum_{j\neq1}^{m} e^{z{\textsubscript{\tiny j}}}))}} = Sigmoid(z{\textsubscript{\tiny i}} - log (\sum_{j\neq1}^{m} e^{z{\textsubscript{\tiny j}}})) 
\end{equation}

Next, using the result from \cite{pant2017smooth}, we approximate \emph{log-sum-exp} as,
\begin{equation}\label{log_max}
log ( \sum_{j=1}^{m} e^z\textsubscript{\tiny{j}}) \approx max_{j\neq1}^{m}
\end{equation}

Using (\ref{sig_as_logsum}) and (\ref{log_max}), we approximate softmax using a max operator and a sigmoid,
\begin{equation}\label{sig_approx}
\sigma (\overrightarrow z){\textsubscript i} \approx Sigmoid(z\textsubscript i - max_{j\neq i}^{m})   
\end{equation}

In other words, the approximated softmax,
\begin{equation}\label{sig_approx2}
 \sigma' (\overrightarrow z){\textsubscript i} = Sigmoid(z\textsubscript i - max_{j\neq i}^{m}) 
\end{equation}

Now that we know the relation know how to implement a softmax using a sigmoid and max, we need to find a piece-wise linear approximation of sigmoid since sigmoid is also an exponential function.

\subsubsection{Approximating sigmoid (Iterative piece-wise approximation)}
We approximate sigmoid as a piece-wise linear function using the Remez exchange algorithm\cite{remez}. The Remez algorithm is an iterative algorithm that finds simpler approximations to functions. It aims to minimize the maximum absolute difference between the approximated polynomial and the actual function. The algorithm starts by taking in the maximum acceptable error $\epsilon$ from the user. It then generates 'L' linear segments to approximate the sigmoid function such that the approximation error is less than $\epsilon$.
We select the initial input domain based on $\epsilon$ and start the Remez algorithm in the domain $(Sigmoid^{-1}(\epsilon), Sigmoid^{-1}(1-\epsilon))$, where $Sigmoid^{-1}$ is the inverse function of the Sigmoid. The inverse of Sigmoid is the logit function i.e., $Sigmoid^{-1}(y)=logit(y)=log (y)/(1-y)$. For example, if the user sets $\epsilon$ to 0.0006, then the input domain for the algorithm lies in (-7.423034723582278, 7.423034723582278)  

%We select (-6.9068, 6.9068) as the input domain (since \emph{Sigmoid}(-6.9068) = 0.00099 and \emph{Sigmoid}(6.9068) = 0.99900, which are very close to 0 and 1 respectively). We start the algorithm with the point (-6.9068,0) and use the Remez exchange algorithm\cite{remez} recursively.  

\subsubsection{Sound approximation}
As stated above, we denote the confidence with which outputs are predicted by $f(\vec{x})$ as $conf(f(\vec{x}))$.  However, softmax being a non-linear activation function cannot be used directly in our case. Hence, we approximate it as a linear function $\sigma'$ (from (\ref{sig_approx2})). We denote this approximated confidence by $conf'(f(\vec{x}))$. Note that $conf'(f(\vec{x})) = \sigma'(f(\vec{x}))$. Also, it is known that,

\begin{equation}\label{lse_bounds}
\begin{split}
max(z_1,\dotsc ,z_n)\leq LSE(z_1,\dotsc ,z_n)\leq max(z_1,\dotsc ,z_n)\\ +log(n)
\end{split}
\end{equation}
Substituting (\ref{lse_bounds}) in  (\ref{sig_approx2}), we get,
$\sigma(z_i,max_{j\neq i}+log(n))\leq \sigma(z_i,LSE)\leq \sigma(z_i,max_{j\neq i})$,
which implies that, \begin{equation}\label{conf_bounds}
\begin{split}
conf'(z_i,max_{j\neq i}+log(n))\leq conf'(z_i,LSE_{j\neq i})\leq \\conf'(z_i,max_{j\neq i})    
\end{split}
\end{equation}
In our implementation, we use the lower bound from equation (\ref{conf_bounds}), i.e. $conf'(z_i,max_{j\neq i}+log(n))$. This means that our (approximated) confidence will always be less than or equal to the exact confidence. For instance, if the approximated confidence is 0.75, the actual confidence will be either greater than or equal to 0.75. This ensures that our confidence approximation is sound.
%Next, applying softmax function to F(x) gives the confidence with which outputs are predicted by N.  We denote this as conf(f(x)). However, softmax being a non-linear activation function cannot be directly used in our case. Hence, we approximate it as a linear function represented as conf'(f(x)), where conf'(f(x)) approximates conf(f(x)).  

\subsubsection{Sound approximation}\label{sound_softmax}
As stated above, we denote the confidence with which outputs are predicted by $f(\vec{x})$ as $conf(f(\vec{x}))$.  However, softmax being a non-linear activation function cannot be used directly in our case. Hence, we approximate it as a linear function $\sigma'$ (from (\ref{sig_approx2})). We denote this approximated confidence by $conf'(f(\vec{x}))$. Note that $conf'(f(\vec{x})) = \sigma'(f(\vec{x}))$. Also, it is known that,

\begin{equation}\label{lse_bounds}
\begin{split}
max(z_1,\dotsc ,z_n)\leq LSE(z_1,\dotsc ,z_n)\leq max(z_1,\dotsc ,z_n)\\ +log(n)
\end{split}
\end{equation}
Substituting (\ref{lse_bounds}) in  (\ref{sig_approx2}), we get,
$\sigma(z_i,max_{j\neq i}+log(n))\leq \sigma(z_i,LSE)\leq \sigma(z_i,max_{j\neq i})$,
which implies that, \begin{equation}\label{conf_bounds}
\begin{split}
conf'(z_i,max_{j\neq i}+log(n))\leq conf'(z_i,LSE_{j\neq i})\leq \\conf'(z_i,max_{j\neq i})    
\end{split}
\end{equation}
In our implementation, we use the lower bound from equation (\ref{conf_bounds}), i.e. $conf'(z_i,max_{j\neq i}+log(n))$. This means that our (approximated) confidence will always be less than or equal to the exact confidence. For instance, if the approximated confidence is 0.75, the actual confidence will be either greater than or equal to 0.75. This ensures that our confidence approximation is sound.

\begin{theorem}
If a class C is predicted by a neural network D with confidence x, then the linearly approximated neural network D' (in SMT) predicts C with confidence x $\pm{y}$, where y is the upper bound to the error introduced by the approximation.  
\end{theorem}

\begin{theorem}
Given a neural network D and an approximation of D, namely, D' with an error $\delta$, if a query Q holds on D', then Q also holds on D. 
\end{theorem}

\begin{theorem}
Let T be an existing sound and complete neural network verification technique that verifies a definition d. Suppose S is a static analysis technique implemented by taking the program product of T and extending it with a softmax function. Then, S verifies a sound over-approximation of d.
\end{theorem}


\begin{theorem}
    Our technique is sound, given that the off-the-shelf static analysis tool used as the solver is sound and complete.
\end{theorem}

\begin{proof}
    From \ref{tm}, we know that $\forall x. \ |\conf(f(x)) - \confabs(f(x))| \leq \gamma_n$, i.e. the actual confidence is greater than the approximated confidence by at most $\gamma_n$. In other words, $\forall x. \conf(f(\vec{x})) \ \geq \ \delta +  \gamma_n \to \conf(f(\vec{x})) \ \geq \ \delta$. Using this result in our specification, we can infer that,
\begin{equation*}
\begin{split} 
\forall x, x'. \ |x-x'| \leq \epsilon \land \conf(f(x)) \geq \delta +  \gamma_n  \land \conf(f(x')) \\
 \geq \delta + \gamma_n   \to class(f(x)) = class(f(x')) \qquad \\ \implies 
 \forall x, x'. \ |x-x'| \leq \epsilon \land \conf(f(x))\\ \geq \delta \land \conf(f(x')) \geq \delta \to class(f(x)) = class(f(x'))
\end{split} 
\end{equation*}

Intuitively, The soundness theorem states that every concrete execution of the neural network is a subset of the abstract executions in the over-approximation.

The fact that our (i) product neural network is sound and complete and (ii) our linearized softmax is sound but not complete because of the over-approximation, proves that our technique is sound if the off-the-shelf static analysis tool used is sound and complete. 

\end{proof}


Consider a  feed-forward neural network, described by a concrete function $f : I \to O$ where $I \in \mathbb{R}^n$ and $O \in \mathbb{R}^m$.
Let the corresponding abstract function be represented as $\hat{f} : \hat{I} \to \hat{O}$.
The connections between concrete and abstract domains are described by a pair of functions such that, $\alpha_I : \mathcal{P}(I) \to \hat{I}$, $\alpha_O : \mathcal{P}(O) \to \hat{O}$ are the abstraction functions and $\gamma_I : \hat{I} \to \mathcal{P}(I), \gamma_O : \hat{O} \to \mathcal{P}(O)$ are the concretization functions. Here, $\mathcal{P}(I)$ and $\mathcal{P}(O)$ are powersets of I and O that describe properties of the concrete domain.

%To establish the soundness of our verification technique, let us begin by recalling the definition of soundness: 
The neural network, $f$ is sound with respect to $\hat{f}$ if the abstract function $\hat{f}$ provides an over-approximation of all the behaviors exhibited by the concrete function f. Formally, $f$ is sound w.r.t. $\hat{f}$ iff

 $$\forall X \in \mathcal{P}(I). \: \: \alpha_O \{f(x) | x \in X\} \subseteq \hat{f}{(\alpha_I(X))} $$

In order to prove that our technique is sound, we need to prove the following: 

The over-approximation in our technique can be introduced by (1) the over-approximated $\hat{f(\vec{x})}$ (due to the linear approximation of $\widehat{softmax}$) and/or (2) the underlying static analysis tool (if the tool is sound but not complete)  

Let us address the first cause: the over-approximated $\hat{f(\vec{x})}$ (due to the linear approximation of $\widehat{softmax}$). From Theorem \ref{tm}, we know that the actual confidence is always greater than the approximated confidence. This means the approximated neural network undergoes a stricter check.

However, since Marabou is sound and complete, we can ignore the 'static analysis tool' aspect. This means that over-approximation in $\hat{f}(\vec{x})$ is introduced only by $\widehat{softmax}$. Thereby, using the definition of soundness, the soundness of  $\hat{f}(\vec{x})$ implies the soundness of f$(\vec{x})$.

\begin{equation}\label{eq_f(x)sound}
      Soundness \:of \hat{f}(\vec{x})  \implies Soundness \:of f(\vec{x}) 
\end{equation}



%\subsubsection{Checking equivalence of output classes} 
% Encoding the consequence, $\class(f(\vec{x}) = \class(f(\vec{x'})$ of our 2-safety property in Marabou is not straight-forward. This is because Marabou does not have an in-built implication operator.  Hence, we had to come up with a workaround to encode this in Marabou. Let $\vec{z}$ and $\vec{z'}$ be the vectors representing the neurons in the last but one layer, where $\vec{z}$ and $\vec{z'}$ correspond to input vectors $\vec{x}$ and $\vec{x'}$ respectively. Now, max($\vec{z}$) and max($\vec{z'}$) give the output classes to which $\vec{x}$ and $\vec{x'}$ are classified. encode the following constraint will ensure that $\vec{x}$ and $\vec{x'}$ are classified to the same output class:
% [$(max(\vec{z}) \ - \ \vec{z_1}) = 0 \ \land \ (max(\vec{z'})  \ - \ \vec{z'_1}) = 0] \ \vee \ [(max(\vec{z})  \ - \ \vec{z_2}) = 0 \ \land \ (max(\vec{z'})  \ - \ \vec{z'_2}) = 0] \ \vee \ \dotsc \ \vee \ [(max(\vec{z})  \ - \ \vec{z_n}) = 0 \ \land \ (max(\vec{z'})  \ - \ \vec{z'_n}) = 0]$, where n is the number of output classes.

% This will check that if $\vec{x}$ is classified as class i then $\vec{x'}$ would also be classified as class i. However, since there was no direct way to encode this in Marabou, for every output class i, we execute a separate query: [$max(\vec{z}) \ - \ \vec{z_1} \ \land \ max(\vec{z'})  \ - \ \vec{z'_1}]$.

First, checking the validity of the implication in \autoref{conf_rob} can be reduced to checking the unsatisfiability of  
\begin{multline}
      ||\vec{x} - \vec{x}'|| \leq \epsilon \ \wedge \conf(f(\vec{x})) \geq \kappa \; \wedge\\ \class(f(\vec{x})) \neq \class(f(\vec{x}'))
\end{multline}

However, the grammar in \autoref{marabou_grammar} provides no means to encode disequality or $\class$ (which returns the {\em index} pointing to the largest element of a vector). To implement disequality, we perform a case split over all $n=\vert V^l\vert$ labels by instantiating  the encoding of the entire network over $\mathsf{out}_{l,i}$ and $\mathsf{out}'_{l,i}$ for $1\leq i\leq n$:
\begin{multline} 
      \ldots\;\wedge\;\overbrace{\max (\mathsf{out}_{l,1},\ldots,\mathsf{out}_{l,n})}^{\conf(f(\vec{x}))} > \kappa\; \wedge \\  
    \left(\max (\mathsf{out'}_{l,1},\ldots,\mathsf{out'}_{l,n})-\mathsf{out'}_{l,i} < 0\right)\;\\
    \vee  \ldots\;\wedge\;\overbrace{\max (\mathsf{out}_{l,1},\ldots,\mathsf{out}_{l,n})}^{\conf(f(\vec{x}))} > \kappa\; \wedge \\  
    \left(\max (\mathsf{out'}_{l,1},\ldots,\mathsf{out'}_{l,n})-\mathsf{out'}_{l,i} > 0\right)
    \label{unsat_class_query}
\end{multline}

The constraint $(\max (\mathsf{out}_{l,1},\ldots,\mathsf{out}_{l,n})-\mathsf{out}_{l,i}=0)$ ensures that $\out_{l,i}$ corresponds to the largest element in $f(\vec{x})$ (and hence that $\class(f(\vec{x})=i$). Moreover, the constraint on $\conf(f(\vec{x}))$ guarantees that $\out_{l,i}\geq (\kappa - b)$. Consequently, if $\out'_{l,i}<(\kappa - b)$ (encoded by the sign constraint), then we can conclude that $\class(f(\vec{x}'))\neq i$ and hence the robustness constraint is violated.

What remains is the case where $\mathsf{out}'_{l,i}\geq (\kappa - b)$ but $\max (\mathsf{out}'_{l,1},\ldots,\mathsf{out}'_{l,n})-\mathsf{out}'_{l,i}>0$. In that case, we know that $\max (\mathsf{out}'_{l,1},\ldots,\mathsf{out}'_{l,n})+\mathsf{out}'_{l,i}\leq 1$ since the last layer represents a probability distribution. Since $\conf(f(x))> (\kappa - b)$ and $\mathsf{out}'_{l,i}\geq (\kappa - b)$, this is only feasible for $\kappa\leq\frac{1}{2}$.

Consequently, we can check for a violation of the robustness property in \autoref{conf_rob} by performing $n$ unsatisfiability queries (\ref{unsat_class_query}) as long as $\kappa>\frac{1}{2}$.

%While the above transformation is equivalence preserving for $\kappa>\frac{1}{2}$, the encoding of \softmax requires an approximation approach (described in the following subsection).

\begin{figure}[h!]
  \centering
  %[width=0.9\linewidth]
  %\includegraphics[width=0.5\textwidth]{my-%uploaded-figure.png}
  \includegraphics[scale=0.58]{images/german_credit_plot}
  \caption{Input distance vs. confidence for German credit dataset}
  \label{fig:german_credit}
\end{figure}

\begin{figure}[h!]
  \centering
  %[width=0.9\linewidth]
  %\includegraphics[width=0.5\textwidth]{my-%uploaded-figure.png}
  \includegraphics[scale=0.58]{images/adult_plot}
  \caption{Input distance vs. confidence for adult dataset}
  \label{fig:adult}
\end{figure}

\begin{figure}[h!]
  \centering
  %[width=0.9\linewidth]
  %\includegraphics[width=0.5\textwidth]{my-%uploaded-figure.png}
  \includegraphics[scale=0.58]{images/law_plot}
  \caption{Input distance vs. confidence for law school dataset}
  \label{fig:law}
\end{figure}

\begin{figure}[h!]
  \centering
  %[width=0.9\linewidth]
  %\includegraphics[width=0.5\textwidth]{my-%uploaded-figure.png}
  \includegraphics[scale=0.58]{images/compas_plot}
  \caption{Input distance vs. confidence for COMPAS dataset}
  \label{fig:compas}
\end{figure}
sat 0.99
real	134m54.140s
user	134m48.268s
sys	0m2.214s

unsat 0.999
real	82m57.368s
user	82m52.415s
sys	0m1.776s

German credit, Adult, Law School and COMPAS datasets. We are able to prove that the neural networks are robust for confidence values above 0.75, 0.5, 0.5 and 0.5 respectively. We also get counterexamples for the neural network trained with the German credit dataset for confidence values below 0.7.


\begin{proof} 
The error bound is the difference between the upper and lower bounds of the $\softmax$ and it is a function of the number of outputs $n$ of the neural network and the error $\delta$ for the approximation of the sigmoid.

%$y = -z_i + max_{j\neq i}(z_1\dotsc z_n)$
\begin{equation*}
\begin{split}
     \gamma(n,\delta,\vec{z})\textsubscript i =
     \Sigmoidapp(z{\textsubscript{\tiny i}} -  \mathop{max_{1}^{n}}_{j\neq i}(z_j)) + \delta -  \widehat{\softmax}  (\vec{z})\textsubscript i 
\end{split}
\end{equation*}
\begin{equation*}
\begin{split}
     \gamma(n,\delta,\vec{z})\textsubscript i = \frac{\alpha(\vec{z}) \textsubscript i  (n -2)}{(\alpha (\vec{z})\textsubscript i +1) ((n-1)\alpha(\vec{z})\textsubscript i + 1)} + 2\delta 
\end{split}
\end{equation*}
where: 
\begin{equation*}
\begin{split}
     \alpha(\vec{z}) \textsubscript i  = e^{-z_i + \mathop{max_{1}^{n}}_{j\neq i}(z_j)}
\end{split}
\end{equation*}

Since $z_i = max(z_1, \cdots, z_n)$ then is always $0 < \alpha(\vec{z}) \textsubscript i  \leq 1 $. 
Let us now replace $\alpha(\vec{z}) \textsubscript i $ with the variable $m$ and study the function in the domain $m \in ]0,1]$ with $n \in \mathbb{N}, n \geq 2$:
\begin{equation*}
\begin{split}
\zeta_n(m) = \frac{m  (n -2)}{((m +1) ((n-1)m + 1)}
\end{split}
\end{equation*}
To compute the maximum in the domain $m \in ]0,1]$ we first compute the derivative using the quotient rule:
\begin{equation*}
\begin{split}
\zeta'_n(m) = \frac{(n -2) ((1-n)m^2 + 1)}{((m +1)^2 ((n-1)m + 1)^2}
\end{split}
\end{equation*}
To find the point $m_{max}$ for which we have the maximum $\zeta_n(m_{max})$, we need to find the positive root for the following equation:
\begin{equation*}
\begin{split}
(n -2) ((1-n)m^2 + 1) = 0
\end{split}
\end{equation*}
The positive root is: 
\begin{equation*}
\begin{split}
m_{max} = \frac{1}{\sqrt{n-1}}
\end{split}
\end{equation*}
As a consequence, the maximum is:
\begin{equation*}
\begin{split}
\zeta_n(m_{max}) = \frac{n-2}{(\sqrt{n-1} + 1)^2} 
\end{split}
\end{equation*}
If the number of outputs is two, the softmax behaves as a sigmoid. Thus, the only error is the one due to the piece-wise approximation ($2 \delta$) of the sigmoid. Let us assume to have three outputs and $\delta=0.0001$ then the maximum error between the real softmax and the approximated one is $\frac{1}{(\sqrt{2} + 1)^2} + 0.0002 \sim 0.17177$.

\end{proof}



\begin{proof} $\conf(\hat{f}(\vec{x}))=\max(\hat{\out}(v_{l,1}),\ldots,\hat{\out}(v_{l,n})) > \frac{1}{2}$. Let us assume that the component $\hat{\out}(v_{l,i}) > \frac{1}{2}$ is the maximum value resulting from applying the approximated softmax. From Theorem 1 we have that $\out(v_{l,i}) \geq \hat{\out}(v_{l,i}) > \frac{1}{2}$ and consequently $i$ is the class for both the real and the approximated neural network $\class(f(\vec{x})) = \class(\hat{f}(\vec{x}))$.

%Let us define a function $h(n) = \frac{1}{n} + \frac{n-2}{(\sqrt{n-1} + 1)^2}$. Using WolframAlpha we can prove analytically that: $$h(n+1) > h(n), \mbox{ for } n\geq 1$$
% Since for $h(2)=\frac{1}{2}$ then $h(n)\geq \frac{1}{2}, \mbox{ for } n\geq 2$ and also 
% $\frac{1}{n} + 2( \frac{n-2}{(\sqrt{n-1} + 1)^2} + 2\delta) \geq h(n) + 2\delta  \geq \frac{1}{2}, \mbox{ for } n\geq 2$.

% Now $\conf(\hat{f}(\vec{x}))=\max(\hat{\out}(v_{l,1}),\ldots,\hat{\out}(v_{l,n}))$. Let assume that the  component $\hat{\out}(v_{l,i})$ is the maximum. From Theorem 1 we have $| \hat{\out}(v_{l,i}) - \out(v_{l,i}) | \leq \frac{n-2}{(\sqrt{n-1} + 1)^2} + 2 \delta$ and from the 
% hypothesis of Theorem 2 we have $\conf(\hat{f}(\vec{x}))=\hat{\out}(v_{l,i}) > \frac{1}{n} + 2( \frac{n-2}{(\sqrt{n-1} + 1)^2} + 2\delta)$. This means that $\out(v_{l,i}) > \frac{1}{n} + ( \frac{n-2}{(\sqrt{n-1} + 1)^2} + 2\delta) \geq \frac{1}{2}$ and consequently $i$ is the class for both the real and the approximated neural network $\class(\hat{f}(\vec{x})) = \class(f(\vec{x}))$.

 \end{proof}



\begin{proof}
    
Let us consider all possible cases around the implications one by one and see if they hold. The theorem to prove is of the form $(\hat{A} \implies \hat{B}) \implies (A \implies B)$ where:
\begin{align*}
&\hat{A} \defn  \left(\forall \vec{x}, \vec{x'}.||\vec{x}-\vec{x'}|| \leq \epsilon \land {\conf}((\hat{f}(\vec{x})) > (\kappa - b_{n,\delta})\right), \\
 &\hat{B} \defn \left({\class}(\hat{f}(\vec{x})) = {\class}(\hat{f}(\vec{x'}))\right) ,\\
&A \defn  \left(\forall \vec{x}, \vec{x'}.||\vec{x}-\vec{x'}|| \leq \epsilon \land \conf(\vec{f(x)}) > \kappa\right), \\
&B \defn  \left(\class(f(\vec{x})) = \class(f(\vec{x'}))\right) 
\end{align*}

Case 1: If ${\conf}(\hat{f}(\vec{x})) \leq \kappa - b_{n,\delta}$ then $\conf(f(\vec{x})) \leq \kappa$ follows from Theorem 1 and the assumption that $\conf(\hat{f}(\vec{x})) > \frac{1}{2}$. $\hat{A}$ will be false and $\neg \hat{A} \implies \neg A$ so also $A$ is false and 
 $(\hat{A} \implies \hat{B}) \implies (A \implies B)$ is true. \\


Case 2: Assume ${\conf}(\hat{f}(\vec{x})) > \kappa - b_{n,\delta}$. From Theorem 2 we have that $\class(\hat{f}(\vec{x})) = \class(f(\vec{x}))$ and $\class(\hat{f}(\vec{x'})) = \class(f(\vec{x'}))$ so $\hat{B} \implies B$ and then independently of $A$ we have that $(\hat{A} \implies \hat{B}) \implies (A \implies B)$ is true.





%This means that if Definition \ref{conf_rob} yields sat/unsat on $\hat{f}(\vec{x})$, it would yield sat/unsat on $f(\vec{x})$.

%%From Theorem \ref{tm}, we know that the actual confidence is greater than the approximated confidence by at most $\frac{n-2}{(\sqrt{n-1} + 1)^2} + 2 \delta $, where n is the number of neurons in the last layer. Let us denote this by $\gamma_{max}(n)$. Then it holds that,

The soundness theorem, thereby, states that if the confidence-based global robustness property holds on the over-approximated neural network, it also holds on the original network. %Intuitively, the theorem states that every concrete execution of the neural network is in the set of  executions of the over-approximated network.
\end{proof}


\begin{comment}
\begin{displaymath}
\begin{aligned}
\forall x = (x_s, x_ns), \; x' = (x'_s, x'_ns)\,.\,
      (x_ns = x'_ns)  \wedge (x_s \neq x'_s) \wedge \conf(f(\vec{x})) > \kappa \implies \\ \class(f(\vec{x})) = \class(f(\vec{x}'))
\end{aligned} 
\end{displaymath}
\end{comment}


\begin{multline*}
(ii) \; \left(\begin{split} \forall \langle x_s, \vec{x}_n\rangle, \; \langle x'_s, \vec{x}'_n\rangle\,.\,
      (\vec{x}_n = \vec{x}'_n)  \wedge (x_s \neq x'_s) \wedge \conf(\hat{f}(\langle x_s, \vec{x}_n\rangle)) > \kappa \implies \\ \class(\hat{f}(\langle x_s, \vec{x}_n\rangle)) = \class(\hat{f}(\langle x'_s, \vec{x}'_n\rangle)) \end{split}\right) \\ \implies 
      \left(\begin{split} \forall \langle x_s, \vec{x}_n\rangle, \; \langle x'_s, \vec{x}'_n\rangle\,.\,
      (\vec{x}_n = \vec{x}'_n)  \wedge (x_s \neq x'_s) \wedge \conf(f(\langle x_s, \vec{x}_n\rangle)) > \kappa \implies \\ \class(f(\langle x_s, \vec{x}_n\rangle)) = \class(f(\langle x'_s, \vec{x}'_n\rangle)) \end{split}\right)
\end{multline*}

==> limitations.tex <==
\section{Limitations}
\label{sec:limitations}

As the error introduced due to the over-approximation of softmax depends on the number of output classes, our approach is limited to neural networks with up to 4 output classes. For neural networks with more than 4 output classes, the error becomes larger and noticeable. We are investing for tighter over-approximations, which will enable us to handle neural networks with a larger number of output classes too. We can handle networks with up to 50 neurons currently. This is due to the overhead of verifying 2-safety in our case vs. 1-safety in the case of Marabou. These constraints suggest potential avenues for guiding further research and remain a part of future work, which we discuss in the next section. 

==> overview.tex <==
\section{Overview}
\label{sec:overview}

This section provides an outline of our approach, motivating our choices and highlighting the challenges.
%

\subsection{Global Robustness with Confidence}

%The intention of robustness properties is essentially to formalize that there should be no adversarial examples, i.e., that the neural network should be robust against small $\epsilon$-perturbations.
%%

Robustness properties aim at specifying that small $\epsilon$-perturbations in a neural network shall not affect and alter the classification results.
Recall the notions of local and global robustness, as introduced in \autoref{background_section}. A violation of these properties is represented by two concrete inputs $\vec{x}$ and $\vec{x}'$ (one of which is given upfront in the context of local robustness). \autoref{fig:overview} illustrates different notions of robustness. 

\autoref{fig:overview}~(a) illustrates the classification of an input $\vec{x}$ that includes two (continuous) features $x_1$ and $x_2$. The pair of purple points is not a counterexample to robustness, as both inputs lie within the same class. The green and blue points, however, represent counterexamples to local (and hence also global) robustness, as they fall on different sides of the decision boundaries. 

%Local robustness is meaningful under certain threat models. 
Local robustness has two major limitations. First,  there are always inputs arbitrarily close to the decision boundary, which then constitute  counterexamples to local robustness. Second, local robustness is defined only for a specific input. Consequently, it does not provide any guarantees for any other input. It follows that the robustness of the entire neural network cannot be assessed with local robustness only. 

We need instead, a global property that evaluates the expected input/output relation over \emph{all} pairs of inputs. To avoid comparing inputs close to decision boundaries, which would lead to a non-satisfiable property,  one can partition the input space based on categorical features,  as typically done for fairness~\cite{khedr2022certifair,BiswasR23} and illustrated in \autoref{fig:overview}~(b). 
Here, we assume that $\vec{x}$ includes a categorical feature $x_3$ in addition to the continuous features $x_1$ and $x_2$. The left (right) part of \autoref{fig:overview}~(b) depicts classes and inputs in the partition based on the categorical feature $x_3$ with value $v$ ($v'$). 
Consequently, only pairs of inputs belonging to the \emph{same} partition are compared. Inputs belonging to two different partitions (e.g. green points in \autoref{fig:overview}~(b)) deviate in at least one categorical feature and can hence be assumed to violate the premise $\|\vec{x}-\vec{x}'\|\leq\epsilon$ of Definition \ref{global_rob}. According to this approach, a classification in a secure network can only change with different categorical values. Any two points that lie in the same partition but belong to different classes (e.g. the pair of blue points in \autoref{fig:overview}~(b)) are considered counterexamples to robustness. This is a strong limitation that does not admit two classes to result from continuous inputs only, as typically required for robustness.

%This is problematic if the line between the two blue points represents a decision boundary, i.e., both of the points are correctly classified rather than being adversarial examples. In particular, the CertiFair approach will classify any pair of sufficiently close input points that agree on their categorical features but are classified differently as counterexamples to robustness.

We address this problem by taking inspiration from the notion of confidence-based robustness for neural networks~\cite{chen2021learning}. We illustrate the intuition of our approach in \autoref{fig:overview}~(c) in which the input space is colored into shades of gray and where every gray value corresponds to a confidence of the network. Darker shades of gray represent higher levels of confidence for the given classification. We consider two reasonable assumptions: (1) continuous inputs can also trigger changes in classification, and (2) the confidence of the neural network at a decision boundary must be relatively low. This is captured by our confidence-based global robustness as it requires that for any input with high-confidence, all its $\epsilon$-neighbour inputs yield the same class (e.g. the two purple points in \autoref{fig:overview}~(c)). Our notion discards inputs near the decision boundaries as counterexamples, as long as they result in outputs with low confidence (e.g. the two blue points in \autoref{fig:overview}~(c)).  Robust systems hence guarantee that input points classified with a high confidence are immune to adversarial perturbation attacks. In \autoref{fig:overview}~(c), the pair of green inputs witness the violation of the confidence-based global robustness -- the two points lie in different classes and one of them has an output with high confidence.

%e consider it a reasonable assumption that at decision boundaries, the confidence for one label gradually decreases whereas the confidence in another one gradually increases. Hence, at the transition point, the confidences in both labels will be lower and close to each other. Hence, we do not consider pairs of inputs whose labels differ, but do so with a low level of confidence, to be counterexamples to robustness. In other words, our confidence-based global robustness property states that for any two input points within a small neighborhood (defined by $\epsilon$) and classified with a high confidence $\kappa$ (e.g., $\kappa=0.98$), the classifier's output should be stable. Hence, this property ensures that inputs near the decision boundary are not considered counterexamples to robustness. Importantly, it also guarantees that input points classified with a high confidence are immune to adversarial perturbation attacks.
%%
We provide a formal definition in \autoref{sec:technical_content} (see Definition~\ref{conf_rob}). 


%
% Existing techniques model properties of neural networks as trace properties, the most common being adversarial robustness. Trace properties are defined as input-output relations of the neural network. The vast majority of existing verification addresses local robustness and fairness properties, which consist in checking whether small perturbations of a specific input can lead to misclassification errors.

%Input-output robustness for a fixed input is a trace property. Since most work on verification aims to tackle adversarial perturbations, which occur for small changes in input, they took on local robustness. Verifying local robustness ensured that small perturbations in the local neighborhood of an input would not lead to misclassification. 
%Formally, a model F is said to be $\delta$-locally-robust at point x if it makes the same prediction on all points in the $\delta$-ball centered at x.
%\begin{definition}[Local Robustness]
%A model, f, is $\epsilon$-locally-robust at point x, if $\forall x' ||x-x'|| \leq \epsilon \to f(x) = f(x')$
%\end{definition}

%Properties that examine pairs or sets of traces are called hyperproperties.  

%Since global robustness holds for all inputs, it is strictly stronger than local robustness and ensures that the system stays robust even under distribution sh

\begin{comment}
begin{figure}[h!]t
  \centering
  %[width=0.9\linewidth]
  %\includegraphics[width=0.5\textwidth]{my-%uploaded-figure.png}
  %\includegraphics[scale=0.38]{images/overview}
  \includegraphics[width=0.7\linewidth]{images/overview.png}
  \caption{(a) Local, (b) partitioned-global and (c) our confidence-based global robustness. $x_1$ and $x_2$ denote continuous input points, while $x_3$ denotes a categorical input in the partitioned-global approach (b). The shades of gray in (c) depict the level of confidence of the neural network with respect to the given inputs -- dark gray denotes high while white denotes low confidence level. The neural network is robust to the pair of purple points in all three cases (a), (b) and (c). The neural network is not robust for the pair of blue points in the case of local and partitioned-global (b) robustness, but is robust according to our definition (c). Finally, the neural network is not robust for the pair of green points according to both the local and the confidence-based global robustness (a) and (c), but is robust with respect to the partitioned-global robustness (b). The global partitioning method does not catch the counterexample, because the two green points are in separate partitions.}
  \label{fig:overview}
\end{figure}
\end{comment}
\subsection{Checking Confidence-based Global Robustness}

In recent years, there has been increased interest and significant advances in static analysis \cite{gehr2018ai2,singh2019abstract,UrbanCWZ20} and automated reasoning techniques \cite{katz2017reluplex, katz2019marabou, khedr2021peregrinn} for neural networks. The first approach essentially treats neural networks as programs, which are then subjected to a static analysis, and the second approach encodes the neural network as a logical formula, which is then checked for satisfiability using automated decision procedures. 

Confidence-based global robustness is  in principle amenable to both approaches. Since it is a 2-safety property, it requires reasoning about \emph{pairs} of such executions. We address this problem by composing~\cite{barthe2011relational} the program\footnote{As executions of feed-forward neural networks are finite, the resulting programs are loop-free.} or formula that represents a given neural network with a copy of itself (cf.\autoref{self_composition}). Consequently, we reduce the problem of checking global robustness to checking a traditional safety property. While this approach is not dependent on a specific verification technique, we demonstrate its applicability by extending Marabou \cite{katz2019marabou}, a state-of-the-art verification tool for neural networks. %This technique essentially amounts to encoding a self-composition of a given neural network as an SMT formula and checking the satisfiability of its negation. Consequently, the resulting instance is satisfiable if (and only if) there is a violation to global robustness with confidence.

\subsection{Approximating Activation Functions and Confidence}

Deploying our confidence-based approach to global robustness in state-of-the-art verification tools like Marabou \cite{katz2019marabou} raises a number of challenges that are specific to the typically limited capabilities of the underlying decision procedure. For instance,  the logical formalism supported by Marabou  does not support negation, which complicates encoding our global robustness property, requiring us to rely on linear arithmetic and the maximum operator instead. Furthermore, it does not support the sigmoid function required to implement the \softmax (final) of our feed-forward neural networks, and this is a limitation shared with the other state-of-the-art verifiers for DNNs. To tackle this problem, we present an approximation of the \softmax function and provide lower and upper bounds for its error. This allows us to encode an over-approximation of the original neural network in state-of-the-art  verification tools like Marabou.  
Finally, we prove that our analysis of the confidence-based global robustness property over the over-approximated network is sound.  

% Figure \ref{fig:intro} illustrates the difference between local (a), partitioned-global (used in CertiFair) (b), and our global definition (c). (a) depicts local robustness property verified on a neural network with 3 output classes (class 1, class 2 and class 3) The black curves denote the decision boundaries of these classes. The local robustness property would check that points very close to a specific input point are classified similarly. So, neither of the black, blue, or orange points will result in a counter-example since they are sufficiently close to each other and assumed to be in the same class. However, as we can see the blue and orange points should have resulted in counter-examples. be class points are classified correctly since they lie in the same class. (b) depicts the partitioned global property, where the blue-dotted squares denote the input partitions. The partitioned-global property checks that all inputs that are close to each other and lie in the same input partition are classified to the same label. This means that a neural network that is robust w.r.t this property is robust for the pair of blue points since they lie in the same partition. It is however not robust for the pair of orange points, since they lie in different partitions and hence would never be compared. (c) illustrates confidence-based global robustness property, where a darker shade of gray represents a higher confidence-score in the label predicted by the neural network. Here, we see that the black points are fine. Second, the confidence-score for the blue points and they would thus result in a counter-example. Finally, the orange points are very close, are classified with high-confidence score and still are in different classes, thereby resulting in a counter-example too, which the local and partitioned-global properties could not catch.  

% Verifying confidence-based global definition is however not trivial. This is because, to obtain confidence, the softmax layer is needed and to the best of our knowledge, no existing static analysis-based neural network verification tool uses it because the softmax layer is very tricky to implement. Softmax is a non-linear function that involves exponentiation and normalization, which makes its implementation in static analyzers challenging. To verify hyperproperties in neural networks, we also need to instrument a model which is amenable to relational verification. 
 
We explain the technical details of our solution in the following subsections.


==> related.tex <==

\section{Related Work}
\label{related}
\textbf{Local robustness.} 
A lot of work has been done in the past decade in the area of neural network verification. Most of the work in literature is guided to tackle adversarial perturbations, i.e. to ensure that similar inputs are not classified to different labels. This led to the research in local robustness verification. There are several SMT-based techniques, \cite{pulina2012challenging}, \cite{huang2017safety}, \cite{li2019analyzing} which encode the neural networks and the property to be verified and use an SMT solver to solve these encodings. The SMT-based techniques are usually precise but take more time. Then there are abstraction-based techniques \cite{pulina2010abstraction}, \cite{singh2019abstract}, \cite{gehr2018ai2}, \cite{10097028} that are not as precise but scale better than SMT-based techniques. In \cite{xu2020fast}, Xu et al. present a complete verifier that uses linear relaxation-based perturbation analysis instead of linear programming.
Abstraction-based techniques typically find an over-approximation of the neural network as a whole, or they might abstract the activation functions. The abstractions are easier to reason about than the original problem which was abstracted. Also, there are techniques which use mixed-integer programming \cite{cheng2017maximum, tjeng2017evaluating, dutta2018output} to certify neural networks. Also, there is Marabou \cite{katz2019marabou}, which we used as our solver and its predecessor Reluplex \cite{katz2017reluplex}. Marabou and Reluplex use a modified simplex algorithm. 

\textbf{Global robustness.}
In addition to CertiFair (discussed in Section \ref{sec:overview}, there has been some work on training certifiable neural networks \cite{leino2021globally} and classifiers other than neural networks \cite{chen2021learning}, \cite{calzavara2022beyond} that satisfy global robustness. These works highlight the advantages of using global robustness over local robustness. The work by Leino et al. is most closely related to ours in terms of underlying approach taken. Leino et al. proposed a new approach using Lipschitz bound to ensure global robustness of neural networks. Their technique involves training neural networks with a special output label, called $\perp$, which is used to signal predictions made on a subset of the feature space that is too close to the decision boundary. This subset is potentially vulnerable to evasion attacks. The notion of global robustness introduced by Leino et al. requires that any two inputs that are close must lead to the same output unless the $\perp$ label is returned for at least one of the inputs. Although our verification technique captures a similar notion of global robustness, their objective is to train robust neural networks while we verify them. Furthermore,  their technique is specific to neural networks that use the $\perp$ label and cannot be used to reason about traditional neural networks. 

%Another recent work, CertiFair \cite{khedr2022certifair} designed a way to verify global individual fairness property of ReLU neural network classifiers using distance-based similarity metrics. They model global individual fairness as a hyperproperty. They start by partitioning the input space using categorical features. Next, they run the verifier within each partition to verify the fairness property. Finally, they count the number of verified partitions. There are a few drawbacks in this method. First, partitioning the input space requires manual intervention and thus is dependent on human expertise. Second, input pairs in different partitions are never compared which makes the method unsound with respect to the global fairness property. 
